Beyond Flatland: A Geometric Take on Matching Methods for Treatment Effect Estimation

Matching is a popular approach in causal inference to estimate treatment effects by pairing treated and control units that are most similar in terms of their covariate information. However, classic matching methods completely ignore the geometry of the data manifold, which is crucial to define a meaningful distance for matching, and struggle when covariates are noisy and high-dimensional. In this work, we propose GeoMatching, a matching method to estimate treatment effects that takes into account the intrinsic data geometry induced by existing causal mechanisms among the confounding variables. First, we learn a low-dimensional, latent Riemannian manifold that accounts for uncertainty and geometry of the original input data. Second, we estimate treatment effects via matching in the latent space based on the learned latent Riemannian metric. We provide theoretical insights and empirical results in synthetic and real-world scenarios, demonstrating that GeoMatching yields more effective treatment effect estimators, even as we increase input dimensionality, in the presence of outliers, or in semi-supervised scenarios.

==> sections/01_intro_OLD.tex <==
\section{Introduction}\label{sec:intro}

% Estimating treatment effects from observational data are everywhere, not only in medice but .... 
% The key problem when estimating treatment effects from observational data is the so-called confounding bias, imbalance between cases and controls
% ----
% Matching is ....
% Given pre-treatment variables, treatment and outcome, the goal is to infer  the effect of the treatment by pair/find a hypothetical twin to each unit/observation.... Finding a suitable pair implies minimizing distance metric... This implies minimizing...
%
% An essential element is which distance to use?
% To pair a singleBut to pair cases to controls, what is the right distance?
%


% \begin{figure}[h!]%htbp]
%   \centering
%   % \begin{minipage}[t]{0.3\textwidth}
%   %   \centering
%   %   \includegraphics[width=\textwidth]{figures/swissroll/image1.png}
%   %   \caption{Assumed causal graph.}
%   % \end{minipage}\hfill
%   \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/swissroll/illustration.png}
%     \caption{\textbf{Key idea of the paper}. We propose a matching method that takes into account the geometry of data.}
%   \end{minipage}
% \end{figure}

%\textit{(First paragraph on importance of TE estimation)} 

% TODO: rephrase, too literal from (Yan et.al, 2024)
Causal inference aims to estimate the causal effect of a treatment or a policy~\citep{pearl_causal_2009}, and has been widely used in a wide range of real-world applications, including medicine~\citep{rosenbaum_optimal_2012, razonable_casirivimab-imdevimab_2021}, public policy~\citep{ben-michael_policy_2023}, epidemiology~\citep{westreich_transportability_2017}, and econometrics~\citep{sekhon_matching_2012}. The gold standard for estimating treatment effect is to perform Randomized Controlled Trials (RCTs), which assign a treatment variable at random within the population of interest. However, RCTs are often costly, unfeasible or unethical to run. An alternative is to estimate treatment effect from observational data.

%However, the fundamental problem of causal inference is that one cannot observe the outcome of both the true and the alternative scenario for the same datapoint (also called factual and counterfactual outcomes).
A fundamental issue in observational studies is the so-called confounding bias~\citep{rubin_causal_2005}, which refers to an imbalance/discrepancy in the distributions of treated and control units, due to the treatment not being randomly assigned to the observed population.
% TODO: Add example
% One possible solution is to find a datapoint that is very similar to the treated unit under study but did not received the treatment.
%  "This is the general idea behind matching whereby each treated subject in the sample data is assigned to one or more subjects from the control group (Stuart, 2010)."
% Matching is one of the most popular techniques in --- and --- to estimate a treatment from observational data.
%
Matching is a well-established approach in causal inference to alleviate confounding bias~\citep{stuart_matching_2010},
%The goal is to estimate the effect of a treatment $T$ on an outcome $Y$
where the goal is to pair suitable control units to each treatment unit (and viceversa) based on the similarity of their covariate information.
%pre-treatment covariates $X$, as shown in Figure~\ref{fig:intro_panel}(a).% which involves the process of pairing treatment units with control units on the basis of their covariate information.
%Matching Method (MM) useful (treatment/control units need to be matched to control/treatment units based on covariate information), shown success in several fields, etc (...) \citep{stuart_matching_2010}.

% O Clivio et.al:  "Matching methods, however, generally suffer from the curse of dimensionality (Abadie and Imbens, 2006a; Roberts et al., 2020), rendering them impractical for many modern highdimensional datasets, such as electronic health records or clinical images."
Traditional matching methods suffer from two main limitations: first, they operate in the space of raw input covariates $\mathcal{X}$ which are noisy and high-dimensional, so it becomes harder to build exact matches~\citep{luo_matching_2017}. Indeed, distances become increasingly meaningless for higher dimensions~\citep{goos_surprising_2001, abadie_large_2006}. Second, observations are assumed to live in Euclidean spaces, overlooking the data manifold's geometry: this may lead to distorted distances, undesired matched units, and imprecise estimates of treatment effects. %(see Illustration~\ref{fig:intro_panel}). % Both issues increase extrapolation bias, Add to theoretical insights?. % MFP: TODO: define manifold
%\citep{goos_surprising_2001, abadie_using_2021, roberts_adjusting_2020}

% \paragraph{On the importance of geometry}

% \begin{itemize}
%     \item Geometric structure is an important bias in ML.
%     \item Structural causal models entail geometric structure, geometric structure reflects causal information. 
%     \item Geometry reflects complexity, functional relationship between different R.V.s.
%     \item In (Dominguez-Olmedo et.al, 2023), the authors show the benefits of accounting for the geometry in the generation of causally-grounded counterfactual explanations for ML classifiers.
%     \item Indeed, Riemannian metrics reflect causal knowledge embedded in a SCM~\cite{dominguez-olmedo_data_2023}.
%     \item \cite{dominguez-olmedo_data_2023} shows that structural causal models (SCM) induce geometric structure Under certain mild conditions, causal structure translates into geometric information captured by data manifolds. They derive sufficient conditions, Notable classes of/common classes of SCMs satisfy such conditions.
%     \item Given a Riemannian metric, we can define distance-based operations (like matching for TE estimation) that are informed by the causal structure.
% \end{itemize}

In this work, 
%we assume that observations are the manifestation of a much smaller set of hidden variables (disease, genetics, environmental factors, etc). For example, a particular disease will influence the content of several medical notes and lab tests, but ultimately, it is the absence/presence of the disease that matters.
we assume that the high-dimensional pre-treatment covariates (confounders) lie on a manifold of much smaller dimensionality, this is the so called \textit{manifold hypothesis}. Such manifold structure arises from underlying causal mechanisms that induce statistical correlations among covariates in a constrained manner~\citep{dominguez-olmedo_data_2023}, as illustrated in Figure~\ref{fig:intro_panel}(b).
%
For example, a sport trainer might want to estimate the effect of a particular training strategy (treatment) on athletes performance (outcome). To estimate such effect using observational data, the trainer might need to adjust for a wide variety of covariates, including height, weight and physiological measurements. Here, two athletes should be more or less similar according to natural differences in their physiology's: ideally, distances should respect the manifold structure
%-- which is generally not the case for Euclidean distance --
(here, anatomical constraints) such that confounding bias in treatment effect estimation can be reduced.  
% TODO: refine example, shorten.
%
%\item \textbf{Objective}: learn geometry-aware latent representation where distances between observations are meaningful, enabling downstream applications such as estimation of treatment effects.
%
%We exploit geometry to capture the intrinsic underlying data structure of the confounders distribution, so that confounding bias can be reduced.
%

We propose \textit{GeoMatching}, a method to estimate treatment effects accounting for the underlying geometry and uncertainty of the data. Instead of working in the space of raw input characteristics, we learn a low-dimensional latent representation together with a latent \textit{Riemannian metric} (a generalization of the Euclidean metric) such that raw distances along the original manifold embedded in the high-dim input space are preserved in the low-dim latent space. We can then leverage those \emph{geometry-aware} distances for matching to estimate treatment effects more accurately, as shown in Figure~\ref{fig:intro_panel}(c-d). The latent representation is a \textit{Riemannian manifold}, where distance between two data points is given by minimum path length along the data manifold. To our knowledge, this work is the first one looking at geometry-aware methods (in a differential geometry sense) for causal inference.

%by performing matching in a latent space according to a Riemannian metric (instead of Euclidean) that preserves the geometry of the data manifold in the original input space.
%
%
%We resort to a Gaussian Process Latent Variable model (GPLVM) to learn a latent representation of input covariates while accounting for the uncertainty in the dimensionality reduction step, which is then accounted for in the learned latent Riemannian metric.
%
% We could use a VAE as well~\cite{arvanitidis_latent_2021}, GPs have two advantages: i) suitable inductive biases for uncertainty estimation as we go away from data manifold, ii) closed-form prior distribution for tensor metric thanks to GPs being closed under linear operators (e.g., derivatives).
%
%Figure~\ref{fig:intro_panel} gives an overview and intuition of the proposed approach. The first row depicts the key underlying assumption of our work, i.e., that causal structure implies geometric data structure.
%The second row illustrates the benefit of using a Riemannian metric (instead of Euclidean) to account for data uncertainty: matched pairs will be faithful to the manifold structure (a), which translates into more accurate (less biased) individual and average treatment effect estimators (d-e).

%\begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}
  \vspace{-0.3cm}
  \begin{center}
    %\includegraphics[width=0.48\textwidth]{birds}
    \includegraphics[width=\textwidth]{figures/intro/panel_geomatching_final_4subfigs.png}
  \end{center}
  \vspace{-0.3cm}
  \caption{\textbf{Key idea of the paper}. We propose \textit{GeoMatching}, a geometry-aware matching method that pairs cases and controls along the manifold of confounders $X$. (a) Assumed causal graph in this work; (b) Different sub-causal graphs for the covariates $X$ induce different geometric data structures; (c) GeoMatching learns a latent Riemannian metric $\G$ (represented as colorbar) which captures the geometric structure and uncertainty of the data, enabling matched pairs to be faithful to the manifold structure.
  %Comparison of Standard matching and GeoMatching (our contribution) in terms of matched units and treatment effect estimation performance.
  (d) Geometry-aware matched samples translates into more accurate estimates of individual treatment effect (ITE) and average treatment effect (ATE).
  %, according to average treatment effect (ATE) absolute error averaged across 5 random seeds. %\textbf{Step 1}: train a latent variable model to learn a latent representation $Z$ and Riemannian metric $\mathbb{E}[\mathbf{G}]$. \textbf{Step 2:} estimate treatment effects by matching units according to geodesic distances along the data manifold.
  \label{fig:intro_panel}}
  \vspace{-0.3cm}
%\end{wrapfigure}
\end{figure}

\paragraph{Contributions} We summarize below the key contributions of ths work:
    \begin{enumerate}
        %\item We propose \textit{GeoMatching}, a geometry-aware matching method that accounts for the underlying data structure of the confounders, leveraging Riemannian geometry.
        \item We introduce \textit{GeoMatching}, a geometry-aware matching method that captures the intrinsic data structure of the confounders leveraging Riemannian geometry, and accounts for data uncertainty with particular robustness to outliers.
        \item We study the bias decomposition of the treatment effect estimator for GeoMatching and posit conditions under which it is expected to improve over standard matching methods.
        \item We empirically show that GeoMatching yields better results compared to other baselines on diverse synthetic and real-world datasets, and outbeats baselines as we increase the input space dimentionality, in the presence of outliers, or in semi-supervised scenarios.% as measured by absolute error of average treatment effect.
    \end{enumerate}

% OLD:
% \subsection*{What are desired properties of a patient embedding?}
% \begin{itemize}
%     \item Reflect invariances faithful to the causal mechanisms. Invariant to certain transformation. \textit{Nota Bene}: Any metric choice implies different assumptions on the data. E.g., rotation and translation invariance for L2-norm; affine (rotation, scaling, or translation) invariance for Mahalanobis distance. In our case, we want invariances that are faithful to the causal mechanisms.
%     \item Able to handle stochasticity and geometry of observational data
%     \item ``Graceful'' behavior as we increase input dimensionality.
%     \item Dependent on downstream task: informative w.r.t the query (e.g., treatment effect for a given drug, ideally we want to compute distances only based on causally-related covariates, that is, when learning the latent representation of X, we do not want to preserve all information that reconstructs X, but instead, only match according to covariates that are causally-related to the outcome).
% \end{itemize}

==> sections/03c_method_geomatching_OLD.tex <==
\subsection{Motivation: Bias Decomposition}\label{sec:bias_decomposition}

As previously, let us consider the covariates $X_\star \in \mathbb{R}^d$ of a treated individual ($T_\star = 1$). Our goal is to estimate the individual treatment effect $\mathrm{ITE}(X_\star) = |\mu_1(X_\star) - \mu_0(X_\star)|$, where $\mu_0(X_\star)$ is unobserved.
%
%As in previous sections, let $X_\star \in \mathbb{R}^d$ be the covariates of an individual exposed to a treatment $T_\star = 1$. Let $\mu_1(x)=\mathbb{E}[Y(1) \given X=x]$ and $\mu_0(x)=\mathbb{E}[Y(0) \given X=x]$ denote the expected outcome with or without treatment. Our object of interest is the individual treatment effect $\mathrm{ITE}(X_\star) = |\mu_1(X_\star) - \mu_0(X_\star)|$.
%
%As stated in Equation~\ref{eq:problem_formulation}, matching requires computing the distance $d(X_\star, X_j)$ between treated unit $X_\star$ and control unit $X_j$.
%
Given a fixed distance metric $d(\cdot,\dot)$, we can solve Equation~\eqref{eq:problem_formulation} and build an ITE matching estimator as follows:
%
%Intuitively, we want to choose the distance that minimizes the \textit{extrapolation bias} of the matching estimator:
\begin{eqnarray}
    \widehat{\mathrm{ITE}}(X_\star; d) = |\mu_1(X_\star) - \mu_0(X_{j^\dagger(d)})| = | \underbrace{\mu_1(X_\star) - \mu_0(X_\star)}_{\mathrm{ITE}(X_\star)} + \underbrace{\mu_0(X_\star) - \mu_0(X_{j^\dagger(d)})}_{\mathrm{Bias}(X_\star; d)} |,
\end{eqnarray}
%
where $\mathrm{Bias}(X_\star; d)$ is the \textit{extrapolation bias} or cost to pay from using $X_{j^\dagger(d)}$ instead of $X_\star$.

In an ideal scenario, we can estimate the treatment effect perfectly, i.e., $\mathrm{Bias}(X_\star; d) = 0$, by finding a control unit $X_{j^\dagger(d)}$ s.t. $d(X_\star, X_{j^\dagger(d)}) = 0$.
%
\textit{Perfect matching} methods aim to recover pre-treatment covariates perfectly, but 
%
% This corresponds to \textit{perfect matching}, whose goal is to recover pre-treatment covariates perfectly:
% \begin{equation}
%     \sum^m_{j=1} w_j X_j = X_\star. %X_{j^{\dagger}} = X_\star.
% \end{equation}
%
in practice, it is often unfeasible to find perfect matches.
%
This becomes a bigger challenge as dimensionality and noise of the covariates increases.
%
When matched units are imperfect,
%, i.e., $d(X_{\star}, X_{j^\dagger}) \geq 0$,
matching estimators need to extrapolate, incurring in a non-zero extrapolation bias:
%$|\mu_0(X_{\star}) - \mu_0(X_j) | \geq 0$. 
\begin{equation}
    d(X_{\star}, X_{j^\dagger(d)}) \geq 0 \quad \Rightarrow \quad \mathrm{Bias}(X_\star; d) = |\mu_0(X_{\star}) - \mu_0(X_{j^\dagger(d)}) | \geq 0.
\end{equation}
For example, if the expected outcome without treatment is linear $\mu_0(x) = \beta x$, we incur a bias $d(X_{\star}, X_{j^\dagger(d)}) \beta$ directly proportional to the distance to the match in covariate space.
%
Let us go back to the question ``Which distance metric $d$ should we choose?''.
%
Intuitively, we want to choose the distance that minimizes the bias of the matching estimator:
\begin{equation}
    d^\dagger = \underset{d}{\text{argmin}} \; \mathrm{Bias}(X_\star; d).\label{eq:min_dist}
\end{equation}

\subsection{Assumptions}\label{sec:conditions}

In this work, we make the following two assumptions.
%
%\paragraph{Manifold hypothesis.}
First, we assume the \textit{manifold hypothesis}, which states that the high-dimensional input covariates $X$ lie near a low-dimensional (non-linear) manifold embedded in the original input space~\citep{whiteley_statistical_2024}.
%
Low-dimensional structure arises due to constraints from physical laws and nature, or in other words, geometry results from the underlying causal mechanisms between different covariates~\citep{dominguez-olmedo_data_2023}, as illustrated in Figure~\ref{fig:intro_panel}B.
%
% Under certain mild conditions, causal structure translates into geometric information captured by data manifolds. Notable classes of SCMs satisfy such conditions, as shown by Dominguez.
%
The manifold hypothesis is satisfied under common classes of Structural Causal Models; examples of data types where it is often fulfilled include image vectors representing 3D objects under different angles and light conditions, phonemes in speech signals, or video streams~\citep{fefferman_testing_2016}.
% The \textit{manifold hypothesis}, states that most naturally occurring datasets lie near a non-linear manifold embedded in the
%original input space~\citep{fefferman_testing_2016, dominguez-olmedo_data_2023}.

%\paragraph{Manifold causal coherence.}
Second, we assume \textit{manifold causal coherence}, i.e., that the expected outcomes $\mu_1(x)$ and $\mu_0(x)$ with and without treatment vary smoothly along the manifold structure of the covariates. As we go away from the data manifold (high uncertainty regions), $\mu_1(x)$ and $\mu_0(x)$ might suffer from discontinuities, potentially yielding unbounded extrapolation bias.
%and there is no guarantees on the extrapolation bias.
Intuitively, this assumption tells us that we expect similar outcomes under similar constraints from nature, as dictated by the underlying causal mechanisms. Back to the Intro example
%Section~\ref{sec:intro}
, we expect athletes with similar anatomical constraints (reflected by distances along the manifold) to respond similarly to different training strategies.

Equipped with these two assumptions, we can show that the \emph{Riemannian distance} $d_{\mathcal{R}}(X_{\star}, X_j)$ along the data manifold minimizes the extrapolation bias of a matching estimator, i.e., $d_{\mathcal{R}}(X_{\star}, X_j)$ is the solution of Equation~\eqref{eq:min_dist}.

\subsection{A Geometric Take on Treatment Effect Matching}
%\paragraph{Key Riemannian Concepts.}
The distance between a treated and control unit can be defined as the length of a curve, as illustrated in Figure~\ref{fig:cartoon_distance}. For example, a Euclidean distance corresponds to the length of a straight line. More generally, if data lies on a manifold $\mathcal{M}$ (potentially curved space), the length of a smooth curve $\gamma: [0,1] \rightarrow \mathcal{M}$ is defined as:
\begin{equation}
    \mathrm{Length}(\gamma) = \int_0^1 \sqrt{\gamma'(t)^T \G(\gamma(t))\gamma'(t) dt},
\end{equation}
where $\gamma'(t) = \frac{d}{dt}\gamma(t)$ denotes the velocity of the curve, and $\G$ denotes a \textit{Riemannian metric}, a smooth function that assigns a symmetric positive definite matrix $\G(x)$ to different locations $x \in \mathcal{M}$.
%
Intuitively, $\G$ encapsulates an infinitesimal notion of distance on manifold $\mathcal{M}$.
%
Standard matching relies on Riemannian metric $\G = I$, resulting in Euclidean distances:
\begin{equation}
    d_{\text{Euclidean}}(X_\star, X_j) = ||X_\star - X_j||^2 = (X_\star - X_j)^T \mathbf{I} (X_\star - X_j).
\end{equation}
Mahalanobis matching methods rely on a constant Riemannian metric $\G = \Sigma$,
%i.e., $d_{\text{Mahalanobis}}(X_\star, X_j) = (X_\star - X_j)^T \boldsymbol{\Sigma} (X_\star - X_j)$.
\begin{equation}
    d_{\text{Mahalanobis}}(X_\star, X_j) = (X_\star - X_j)^T \boldsymbol{\Sigma} (X_\star - X_j).
\end{equation}

The \textit{Riemannian distance} $d_{\mathcal{R}}(X_\star, X_j)$ generalizes the Euclidean and Mahalanobis distance by replacing the constant covariance matrix $\mathbf{I}$ or $\boldsymbol{\Sigma}$ by an input-dependent covariance matrix $\G(x)$.
%
The \textit{Riemannian distance} between two points on manifold $\mathcal{M}$ is defined as the length of the \textit{geodesic curve}, which is the length-minimizing curve connecting those two points along the manifold.

%as illustrated in Figure~\ref{TODO:Add}.

%A Riemannian metric $\G$ encapsulates an infinitesimal notion of distance on a manifold $\mathcal{M}$.
%
%More formally, $\G$ defines at each point $x \in \mathcal{M}$ a smoothly varying inner product in the tangent space $T_x\mathcal{M}$. The inner product is defined as:
% \begin{equation}
%       \langle x_1,x_2 \rangle_x = x_1^{\mathrm{T}}\G(x)x_2,
% \end{equation}
% where $x_1, x_2 \in T_x\mathcal{M}$ and $x \in \mathcal{M}$.

% \begin{theorem}
%     Let $\mathrm{Bias}(j)$ be the extrapolation bias of a nearest neighbor matching estimator.
%     %If the manifold hypothesis and manifold causal coherence are satisfied,
%     Under the assumptions of the manifold hypothesis and manifold causal coherence,
%     matching treated and control units according to the Riemannian distance $d_{\mathcal{R}}(X_{\star}, X_j)$ minimizes $\mathrm{Bias}(j)$.\label{theorem}
% \end{theorem}

% \begin{proof}
% Here is the proof, seems very intuitive, todo: translate into math notation. Lipschitz argument. todo: complete.
% \end{proof}

%Lower bound the absolute ATE error computed in the original covariate space by absolute ATE error computed in latent Riemannian manifol03_d

%Differential geometry enables us to compute distances in a given space following data structure.

 %Given a treated and control units, what is the best distance metric $d$ to compare them?
 %
% This is a crucial question in matching, and the choice of the distance differs between common matching techniques.
%
% As discussed in previous Section, the default choice is to use Euclidean distances .... However, if the considered space is not Euclidean (i.e., data lying on a curved space), Euclidean distances might not reflect meaningful similarity.

%Why does accounting for geometry yield benefits? Because often lives in a manifold, and methods that account for geometry rely on more meaningful notions of distances. 

%
%Motivated by the manifold hypothesis and the success of geometry-aware models in the machine learning community, we propose GeoMatching, an approach for treatment effect estimation that takes into account the intrinsic geometry and uncertainty of the confounders.
 %
 %In the following we will first introduce and motivate key Riemannian concepts (linking to the matching literature), describe the algorithm, and finally study the bias decomposition of GeoMatching to identify conditions for which GeoMatching is expected to outperform more conventional matching techniques.

\subsection{Algorithm Description}\label{sec:livm}

Under the manifold hypothesis and manifold causal coherence stated in Section~\ref{sec:conditions}, and in addition to the standard causal assumptions of non-hidden confounders, consistency, ignorability and overlap), choosing the Riemannian distance yields better estimation of treatment effects compared to any other distance metric, including the Euclidean distance at the core of the standard matching method. We can now introduce GeoMatching, a geometry-aware matching framework that leverages Riemannian distances to pair treated and control units:
% , summarized in Algorithm~\ref{alg:geomatching}.

%\item \textbf{Step 1}: Learn Riemannian metric $\mathbf{G}$ in a latent space $\mathcal{Z}$ given confounders $X \in \mathcal{X}$.
\paragraph{Step 1: Learn latent Riemannian manifold.} GeoMatching learns a topology-preserving low-dimensional data representation $Z \in \mathcal{Z}$ and latent Riemannian metric $\mathbf{G}$ given confounders $X \in \mathcal{X}$. Considering a latent representation instead of the original input space makes it easier for metric learning, specially if the input space is high-dimensional, and enables to filter out irrelevant information unrelated to the geometry of the confounders. Several methods can be adopted for this stage. Examples are  linear projections with using Principal Component Analysis (PCA)\footnote{Note that PCA is not guaranteed to preserve geometric structure in general, for which other algorithms such as Isomap might be more suitable.} and fitting a kernel-based Riemannian metric $\mathbf{G}$ or training a probabilistic latent variable model to jointly learn $Z$ and $\mathbb{E}[\mathbf{G}]$, propagating Jacobian information. % by propagating Jacobian information, via the pull-back metric.
In the experimental section we resort to \textit{Example Strategy 1}, and posit a parametric Local Inverse Variance (LIV) Riemannian metric~\citep{arvanitidis_locally_2016}, which is defined as the inverse of a local diagonal covariance matrix with entries:
\begin{equation}
    \G_{dd}(x) = \left(\sum_{i=1}^N w_i(x) \left(x_{id} - x_d \right)^2 + \rho \right)^{-1}, \quad \text{where} \quad w_i(x) = \mathrm{exp} \left( -\frac{||x_n - x||^2}{2 \sigma^2} \right).
    \label{eq:livm}
\end{equation}
% TODO: Explain role of sigma and rho in the metric.
%
LIV assumes a locally Euclidean metric, which is then regularized to have large volume measure in regions of the feature space far away from observations. The inductive bias underlying such metric is that shortest paths on the data manifold should remain close to the observed data, we want curves to avoid crossing low-density high-uncertainty regions. A key advantage of this metric is that geodesic computation is less costly, as off-diagonal terms in metric $\G$ are zero.


% Arvanitidis 2022: "The non-parametric space is constructed using a local metric that is the inverse of a local covariance matrix. Here locality is defined via a Gaussian kernel, such that the manifold learning can be seen as a form of kernel smoothing. This indicates that our scheme for learning a manifold might not scale to high-dimensional input spaces".


% Interpretation of locally Euclidean metric in Z space: the intuition is that similarity of observations should be measured based on similarity of their latent variables, in a locally Euclidean sense.

% LVI metric is a deterministic manifold, we also consider a stochastic/statistical manifold...

\paragraph{Step 2: Compute Riemannian distances.} We compute geodesic or Riemannian distances in the latent representation between treated and control units:
\begin{equation}
 d_{\mathcal{R}}(X_{\star}, X_j)  =  \underset{\gamma_j}{\text{min}} \; \mathrm{Length} \Big( f \big(\gamma_j(r) \big); \mathbf{G} \Big),
 \label{eq:geodesic_distance}
\end{equation}
where $\gamma_j: [0,1] \rightarrow \mathcal{X}$ is a curve connecting two datapoints, %the unit of interest $X_\star$ with datapoint $X_j$,
i.e., $\gamma_j(0)=X_{\star}, \, \gamma_j(1)=X_{j}$.
%
To compute geodesic distances, we instantiate a parametrized (discretized) geodesic curve\footnote{Considering a discretized curve for the geodesic scales more gracefully than other graph-based approaches, as the discretization of the curve is always one-dimensional independently of the dimension of the latent space.} and optimize its parameters by minimizing the following second-order ordinary differential equation~\citep{do_carmo_riemannian_1992}:
\begin{equation}
    \gamma'' = -\frac{1}{2}\G^{-1} \left[ \frac{\partial \, \mathrm{vec} \, \G}{\partial \, \gamma} \right]^T (\gamma' \otimes \gamma'),
\end{equation}
where $\mathrm{vec}\, \G$ stacks the columns of $\G$ and $\otimes$ denotes the Kronecker product. Based on Picard-Lindelöf theorem~\citep{tenenbaum_ordinary_1985}, geodesics are guaranteed to exist and are locally unique given a starting point and initial velocity $\gamma'$. 

\paragraph{Step 3: Matching along Riemannian manifold.} Given the Riemannian distances from Equation~\ref{eq:geodesic_distance}, we match treated and control units along the Riemannian manifold by minimizing:
\begin{equation}
    j^{\star} = \underset{j \in [m]}{\argmin} \; d_{\mathcal{G}}(X_{\star}, X_j).
    \label{eq:matching} 
\end{equation}

\paragraph{Step 4: Estimate causal treatment effects.} Given the matched units $\hat{Y}^{\text{match}}_\star$, we can estimate the individual and average treatment effects as follows:
\begin{equation}
    \widehat{\mathrm{ITE}}(X_\star) = Y_\star - \hat{Y}^{\text{match}}_\star, \quad\qquad \widehat{\mathrm{ATE}} 
    %= \mathbb{E}_{X_\star \sim \mathcal{D}} \left[ \mathrm{ITE(X_\star)}  \right]
    = \frac{1}{N} \sum^N_{i=1} \left( Y_\star - \hat{Y}^{\text{match}}_\star \right)\label{eq:te_estimation} 
\end{equation}

% \begin{equation}
%     \widehat{\mathrm{ATE}} 
%     %= \mathbb{E}_{X_\star \sim \mathcal{D}} \left[ \mathrm{ITE(X_\star)}  \right]
%     = \frac{1}{N} \sum^N_{i=1} \left( Y_\star - \hat{Y}^{\text{match}}_\star \right)
%     \label{eq:ate_estimation} 
% \end{equation}

% \paragraph{Option 2: Gaussian Process Latent Variable Model}
% $\mathbf{G} \sim \mathcal{W}_K \left(D, \Sigma_J,  \mathbb{E}[\mathbf{J}^\transpose] \mathbb{E}[\mathbf{J}] \right)$ is a Wishart process with $D$ degrees of freedom and non-centrality matrix $\Sigma^{-1}_J \mathbb{E}[\mathbf{J}^\transpose] \mathbb{E}[\mathbf{J}]$.
% \begin{equation}
%     \mathbb{E}[\mathbf{G}] = \mathbb{E}[\mathbf{J}^\transpose] \mathbb{E}[\mathbf{J}] + D \boldsymbol{\Sigma}_J.
% \end{equation}
% While elegant, this option did not work well in practice, see Appendix for details, etc


%  For each treated unit $X_{\star}$, GeoMatching finds the control unit that minimizes the geodesic distance $d_{\mathcal{G}}(X_*, X_j)$.
% \begin{equation}
%      d_{\mathcal{G}}(X_{\star}, X_j)  =  \underset{\gamma_j}{\text{min}} \; \mathrm{Length} \Big( f \big(\gamma_j(r) \big); \mathbf{G} \Big), 
% \end{equation}
% where $\G$ is a latent Riemannian metric and $\gamma_j: [0,1] \rightarrow \mathcal{X}$ is a curve connecting two datapoints, %the unit of interest $X_\star$ with datapoint $X_j$,
% i.e., $\gamma_j(0)=X_{\star}, \, \gamma_j(1)=X_{j}$.

% \begin{equation}
%     \underset{j \in [m]}{\argmin} \; d_{\mathcal{G}}(X_{\star}, X_j)
% \end{equation}

%Geodesic curve $\gamma^\star_j = \underset{\gamma_j}{\textrm{argmin}} \; \mathrm{Length} \Big( f \big(\gamma_j(r) \big); \G \Big)$

% \begin{algorithm}
%     %\renewcommand\thealgorithm{}
%     \caption{\textit{GeoMatching}: Geometry-Aware Matching Method for Treatment Effect Estimation}
%     \label{alg:geomatching}
%     \textbf{Inputs:} $X \in \mathcal{X}$ (covariates), $T \in \mathbb{Z}$ (treatment), $Y \in \mathcal{Y}$  (outcome), $\mathcal{D} = \{(X_i, T_i, Y_i)\}^N_{i=1}$ (dataset)
     
%      \textbf{Outputs:} $\{X_{j^\dagger} \}$ (matched units for each covariate $X_{\star}$), $\widehat{ITE}$, $\widehat{ATE}$ (treatment effect estimators)
     
%     \textbf{Assumptions:}
%     \begin{itemize}
%         \item \textit{Manifold hypothesis}: confounders $X$ lie on a manifold $\mathcal{M}$.
%         \item \textit{Manifold causal coherence}: outcome models $\mu_1(x)$, $\mu_0(x)$ vary smoothly along $\mathcal{M}$.
%     \end{itemize}

%     \vspace{0.1cm}
    
%     \begin{algorithmic}[1]  % Add line numbers
%         %\Require $n \geq 0$
%         %\Ensure $y = x^n$
%         \STATE Learn latent representation $Z \in \mathcal{Z}$ equipped with Riemannian metric $\mathbf{G}$ given confounders $X$.
%         \FORALL{$X_\star$ in $\mathcal{D}$}
%             \STATE Compute geodesic distances according to Equation~\eqref{eq:geodesic_distance}.
%             \STATE Find best match along Riemannian manifold according to Equation~\eqref{eq:matching}.
%             %\STATE Estimate individual treatment effect %\Comment{This is a comment}
%         \ENDFOR
%         \STATE Estimate individual and average treatment effects according to Equation~\eqref{eq:te_estimation}.
%     \end{algorithmic}
%     %\addtocounter{algorithm}{-1}
% \end{algorithm}

==> sections/07_trash.tex <==
%This section introduces \emph{GeoMatching}, a matching framework for treatment effect estimation that takes into account the intrinsic geometry and uncertainty of the confounders.
%
% Geometry is an important inductive bias in ML and has been shown to yield benefits in diverse applications such as classification, interpolation, model training or synthetic data generation.
%
%Why should we care about data geometry? Manifold hypothesis (explain).
%
% More recently, \cite{dominguez-olmedo_data_2023} has shown that geometry  arises naturally from structural causal models. A natural question is then to explore the benefit of exploiting geometric information in causal inference. To the extent of our knowledge, this work is the first one looking at geometry-aware methods (in a differential geometry sense) for causal inference.

\subsubsection{Gaussian Process Latent Variable Models}

\begin{equation}
    \underset{Z,\lambda}{\text{argmax}} \; p(X \given Z, \lambda)
\end{equation}

\paragraph{Geometrically-informed Regularization-term}

\begin{itemize}
    \item \textbf{Option 1}: Isomap prior for geodesic distances:
    \begin{equation}
        R(\lambda, w) = \frac{1}{S} \sum^S \left(d_{\mathcal{G}}(X_{s_i}, X_{s_j}; \lambda, w) - d_{\text{isomap}}(X_{s_i}, X_{s_j}) \right)^2
    \end{equation}
    \begin{equation}
        R(\lambda, w) = \frac{1}{S} \sum^S \frac{ \left(d_{\mathcal{G}}(X_{s_i}, X_{s_j}; \lambda, w) - d_{\text{isomap}}(X_{s_i}, X_{s_j}) \right)^2 }{d_{\mathcal{G}}(X_{s_i}, X_{s_j}; \lambda, w)^2}
    \end{equation}
    \item \textbf{Option 2}: Ratio of geodesic distances:
    \begin{equation}
        R(\lambda, w) = \frac{\sum_{s \in \mathcal{S}_{\text{near}}} d_{\mathcal{G}}(X_{s_i}, X_{s_j}; \lambda, w)}{\sum_{s \in \mathcal{S}_{\text{far}}} d_{\mathcal{G}}(X_{s_i}, X_{s_j}; \lambda, w)}
    \end{equation}
    \item \textbf{Option 3}: Contrastive (Info-NCE) loss with geodesic distances playing the role of logits. 
    Idea: tell apart which curve corresponds to the true match vs other curves.
    %Idea: tell apart curves that follow manifold from curves that cross-over/step out of the manifold. Let $C_i \in {0,1}$ indicate whether curve $\gamma_i$ belongs to manifold or not.We want to tease out true match from other possible matches.
    \begin{eqnarray}
        R(\lambda, w) = \mathbb{E}_{(X_{\star},X_{\dagger}) \sim \mathcal{S}} \left[ \log \frac{d_{\mathcal{G}}(X_\star, X_\dagger)}{\sum_{X_j \in \mathcal{X}_{\text{controls}} d_{\mathcal{G}}( X_\star, X_j)} }\right],
    \end{eqnarray}
    where $\mathcal{S}$ is the set of tuples such that $X_\star \sim \mathcal{X}_\text{cases}$ and $X_\dagger$ is the corresponding best match according to an oracle.
\end{itemize}

\begin{eqnarray}
        R(\lambda, w) = \mathbb{E}_{(X_{\star},X_{\dagger}) \sim \mathcal{S}} \left[ \log \frac{d_{\mathcal{G}}(X_\star, X_\dagger)}{\sum_{X_j \in \mathcal{X}_{\text{controls}} d_{\mathcal{G}}( X_\star, X_j)} }\right] \approx \log d_{\mathcal{G}}(X_\star, X_\text{pos}) - \log d_{\mathcal{G}}( X_\star, X_\text{neg})
    \end{eqnarray}

==> sections/packages.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors

\usepackage{hyperref}
\usepackage{url}
\usepackage{amsfonts}
\usepackage{setspace}
\usepackage{amsmath}
\usepackage{url}
\usepackage{graphicx}
\usepackage{booktabs}
%\usepackage{multirow}
\usepackage{wrapfig}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{booktabs}
\newtheorem{remark}{Remark}[section]
\usepackage[thinc]{esdiff}
\usepackage{natbib}

\usepackage{tikz}
\usetikzlibrary{bayesnet}
\usetikzlibrary{arrows}
\usepackage{color}
\usetikzlibrary{backgrounds}

%\documentclass{article}
\usepackage{graphicx} % Required for inserting images

\usepackage{paralist}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{mathtools}
\usepackage{bbm}
\usepackage{xcolor}
\usepackage{hyperref}
%\usepackage{algorithmic}
%\usepackage{subfigure}
\usepackage{caption}
%\usepackage{subcaption}
%\usepackage{subfig}
\usepackage{enumitem}
\usepackage{amsmath}
\usepackage{wrapfig}

\usepackage{tikz}
\usetikzlibrary{bayesnet}
\usetikzlibrary{arrows}
\usepackage{color}
\usetikzlibrary{backgrounds}

\usetikzlibrary{shapes,arrows,fit,chains,matrix}
\usetikzlibrary{positioning, shapes.geometric}
\tikzstyle{node_no_draw} = [circle, minimum size = 10mm]
\tikzstyle{node} = [circle, minimum size = 10mm, draw =black!80]
\tikzstyle{nodeinter} = [rectangle, minimum size = 10mm, draw =black!80, fill=gray!30]
\tikzstyle{nodeinterwhite} = [rectangle, minimum size = 10mm, draw =black!80]
\tikzstyle{nodeobserved} = [circle, minimum size = 10mm, draw =black!80, fill=gray!30]
\tikzstyle{box} = [rectangle, draw =black!0]
\tikzstyle{arrow} = [thick,->,>=stealth,line width=0.3mm]
\tikzstyle{arrow2} = [dashed,->,>=stealth,line width=0.6mm]

\usetikzlibrary{calc}
\makeatletter
\tikzset{
  prefix after node/.style={
    prefix after command={\pgfextra{#1}}
  },
  /semifill/ang/.store in=\semi@ang,
  /semifill/ang=0,
  semifill/.style={
    circle, draw,
    prefix after node={
      \typeout{aaa \semi@ang}
      \let\nodename\tikz@last@fig@name
      \fill[/semifill/.cd, /semifill/.search also={/tikz}, #1]
        let \p1 = (\nodename.north), \p2 = (\nodename.center) in
        let \n1 = {\y1 - \y2} in
        (\nodename.\semi@ang) arc [radius=\n1, start angle=\semi@ang, delta angle=180];
    },
  }
}

\usepackage{amsthm}
\newtheorem{definition}{Definition}

\usepackage{multirow}
\usepackage{booktabs}

\usepackage{algorithm}
\usepackage{algpseudocode}

% \newtheorem{theorem}{Theorem}
% \newcommand{\mytheorem}[1]{\par\noindent{\bfseries #1.} \ignorespaces}
% \newcommand{\endmytheorem}{\par}

\usepackage{enumitem}

